Detecting unanticipated mutual recursion using Elegant Objects representation of object-oriented programs

Elegant Objects (EO) is a variation of the object-oriented programming paradigm that favors pure objects and decoration. EO programming language is based on these ideas and has been suggested by Bugayenko as an intermediate representation for object-oriented programs. This paper provides plausible representations in EO of some class-based constructions from Java, C++, and Python. We then reformulate the classical fragile base class problem in the context of these representations. Finally, we discuss an algorithm for detecting a subset of fragile base class patterns in EO programs. We show that using EO as an intermediate language is plausible and discuss possible improvements to the language to assist in richer static analysis.

==> sections/5-detecting-unjustified-assumptions.tex <==
\section{Detecting unjustified assumptions in subclasses}
\label{section:detecting-unjustified-assumptions}

To be done.

\subsection{Inlining method definitions}

To be done. 

\subsection{Keeping track of pre-conditions}

To be done.

\subsection{Detecting fragile overriding}

To be done.

\subsection{Examples}

To be done.


